Large-Scale, Precision Xenon Doping of Liquid Argon

The detection of scintillation light from liquid argon is an experimental technique key to a number of current and future nuclear/particle physics experiments, such as neutrino physics, neutrinoless double beta decay and dark matter searches. Although the idea of adding small quantities of xenon (doping) to enhance the light yield has attracted considerable interest, this technique has never been demonstrated at the necessary scale or precision. Here we report on xenon doping in a 100 l cryogenic vessel. Xenon doping was performed in four concentrations of 1.00$\pm$0.06 ppm, 2.0$\pm$0.1 ppm, 5.0$\pm$0.3 ppm, and 10.0$\pm$0.5 ppm. These measurements represent the most precise xenon doping measurements as of publishing. We observed an increase in average light yield by a factor of 1.92$\pm$0.12(syst)$\pm$0.02(stat) at a dopant concentration of 10 ppm.

==> Extrapolation.tex <==
\section{Extrapolation}
\label{sec Extrap}

In order to understand the effects of xenon doping on a large scale experiment, several optical maps were created for a LEGEND-200 geometry. The current optical design can be seen in Figure \ref{fig 14StringTake2}. The exterior array has a length of $\sim$ 1500 mm and has 1620 fibers placed in a 60 sided polygon with 27 fibers per side. The interior array has a length of 1300 mm and has 936 fibers placed in a 36 sided polygon with 26 fibers per side. An  optical heat map of this geometry with pure liquid argon can be seen in Figures \ref{fig 14StringFiberShroudMapXY} and \ref{fig 14StringFiberShroudMapRZ}. An attenuation length of 60.0 cm was used.

\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=1.\linewidth]{./Figures/Simulations/14StringFiberShroudMapTake2.png}
\caption{ CAD drawing of current 14 string geometry.} 
\label{fig 14StringTake2}
\end{figure}

\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=1.\linewidth]{./Figures/Simulations/14StringFiberShroudMapXY.png}
\caption{ XY projection of optical heat map for current 14 string geometry.} 
\label{fig 14StringFiberShroudMapXY}
\end{figure}

\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=1.\linewidth]{./Figures/Simulations/14StringFiberShroudMapRZ.png}
\caption{ RZ projection of optical heat map for current 14 string geometry.} 
\label{fig 14StringFiberShroudMapRZ}
\end{figure}

==> data.tex <==
\section{data}
This section describes the data that was used to validate the gas doping techniques outlines above as well as two distinct xenon doping data sets. One data set was used to monitor the stability of the xenon mixture as the concentration increased from 0 ppm to 10 ppm, while the other data consists of double coincident cosmic muon interactions.

\subsection{Gas Doping}

In order to validate the gas doping and recirculation system, one small quantity of nitrogen was injected using the methods mentioned in Section \ref{section experiment}. This validation step was done prior to xenon doping because nitrogen can be filtered out using the getter while xenon cannot. Additionally, it would be desirable to show that the doping system can insert a known amount of gas with reasonable uncertainty (less than 10 \%). Past xenon doping experiments such as \cite{CGWahl} have had very large uncertainty ($\sim$50\%) on the amount of xenon inserted and BACoN's doping system should be able to do better than that. 

The effects of nitrogen on argon scintillation light are well known and have been characterized by \cite{triplet1.26} and \cite{Himi:1982hf}. The relationship between the measured triplet life time $\tau'$ and the true triplet life time $\tau$ is dictated by a Birk's law type function:
\begin{equation}
\label{birks law}
    \tau ' = \frac{\tau }{1 + \tau \cdot k \cdot C}
\end{equation}
where $k$ is Birk's constant and $C$ is the molar concentration of impurities measured in parts per million. Birk's constant has been measured to be 0.11 ppm$^{-1} \mu$s$^{-1}$ and $0.13$ ppm$^{-1} \mu $s$^{-1}$ for nitrogen in liquid argon by the two previously mentioned authors. Before moving on, it must be made clear that these previous measurements measured a pure triplet lifetime of 1260 $\pm$ 10stat $\pm$ 55syst ns compared to the  $1479 \pm 38$(stat) $\pm 23$(syst) ns measured in BACoN. The authors \cite{triplet1.26} speculate the difference between what they measure (1260 ns) and what the authors of \cite{triplet1.46} measure (1460 ns) (and what was measured in BACoN) could be explained by different fitting methods and additional impurities in their \say{pure} argon. Authors of \cite{triplet1.26} speculate that if they used the same fitting method used by \cite{triplet1.46} and extrapolate their triplet using equation \ref{birks law} to pure liquid argon, their triplet value becomes 1453 $\pm$ 10stat ns which is in good agreement with the triplet life time measured with BACoN. 

Before any doping is performed, the recirculation and purification system is run and the triplet life time is measured frequently. Once the triplet life time is stable, it is assumed that the pure argon is achieved. Nitrogen contaminant is inserted into BACoN and the triplet lifetime decreases according equation \ref{birks law}. As the argon is purified, it is assumed that the contamination concentration decreases as:
\begin{equation}
    C(t) = C_0 \cdot e^{\sfrac{-t}{\tau_{filter}}}
\end{equation}
where $C_0$ is the initial concentration measured in molar parts per million and $\tau_{filter}$ is a fit parameter.
 
\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=1.\linewidth]{./Figures/GasDoping/BirksDrop.png}
\caption{ Triplet lifetime ($\mu$s) versus run time (days) before and after the nitrogen injections. It can be seen that the nitrogen thoroughly mixed after about three hours.} 
\label{fig BirksDrop}
\end{figure}

 One nitrogen doping run was performed during the duration of the experiment. 1.06 $\pm$ 0.04 ppm of nitrogen were injected into the system. The triplet dropped from 1.479 $\mu s$ to 1.239 $\mu s$ as seen in the Figure \ref{fig BirksDrop}. From this reduced triplet lifetime, a Birk's constant of 0.122 $\pm$ 0.012 $ppm^{-1}\mu s^{-1}$ is found and is consistent with what was measured by the previous two results mentioned above. Using this measured value of Birk's constant, Equation \ref{birks law} was fit to the triplet purification curve. Initial measurements of the filtration time constant found it to be 9.54 $\pm$ 0.55 days (left plot in Figure \ref{fig BirksFit}). It was postulated that the argon was too stable and that the warm pure argon gas was not mixing adequately with the liquid. To increase the filtration rate, the turbo pump was removed from the guard vacuum and the roughing pump was left on, decreasing the insulating vacuum from $5.0\times 10^{-7}$ torr to $1.4\times 10^{-3}$ torr and the coldhead set point was raised from -190 Celsius to -187 Celsius thus increasing the internal pressure of the cryostat from 550 torr to 640 torr. A modification to Equation \ref{birks law} was made to account the for non-zero start time to obtain:
 \begin{equation}
\label{birks lawMod}
    \tau ' = \frac{\tau ' }{1 + \tau ' \cdot k \cdot C_{0} \cdot e^{\sfrac{-(t-t_{0})}{\tau_{filter}}}}
\end{equation}
where $t_{0}$ is the non zero start time of the fit. The filtration time constant measured by fitting Equation \ref{birks lawMod} to the triplet purification curve after these changes was measured to be 4.487 $\pm$ 0.31 days (left plot in Figure \ref{fig BirksFit}).

From the first fit, using the measured Birk's constant, an initial concentration of 1.13 $\pm$ 0.02 ppm was obtained and the second fit yields an initial concentration of 1.09 $\pm$ 0.14 ppm. Both values are consistent with the initial concentration measurement of 1.06 $\pm$ 0.04 ppm.

 
\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=0.49\linewidth]{./Figures/GasDoping/BirksFit1.png}
\includegraphics[width=0.49\linewidth]{./Figures/GasDoping/BirksFit2.png}
\caption[ Nitrogen doping in pure liquid argon for Run Two]{ Nitrogen doping in pure liquid argon for Run Two. The top plot shows the fit obtained when the heat leak for the system was minimized, yielding a filtration rate of 9.541 $\pm$ 0.55 days. The bottom plot shows the fit obtained when a heat leak was added to the system, yielding a filtration rate of 4.487 $\pm$ 0.31 days.} 
\label{fig BirksFit}
\end{figure}
 
 The scintillation distributions for both nitrogen concentrations (0 ppm and 1 ppm) can be seen in Figure \ref{fig MuonPeakLAr}. Both distributions are normalized and then scaled by the max value of the 0 ppm nitrogen measurement which is the maximum amplitude of the singlet. By monitoring the muon peak in the random trigger data before and after doping, as described later in Section \ref{sec XeD}, it is found that the most probable value (MPV) shifts from 334$\pm$7(syst)$\pm$1(stat) PE to 283$\pm$7(syst)$\pm$1 (stat) PE
(Figure \ref{fig MuonPeakLAr}) which corresponds to a 15.3$\pm$3.1\% drop. This drop is compatible with what the authors of \cite{triplet1.26} measure when looking at the total quenching of the waveform from a Cobalt-60 gamma source. 
 
\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=0.49\linewidth]{./Figures/GasDoping/IntensityQuenchingLAr.png}
\includegraphics[width=0.49\linewidth]{./Figures/GasDoping/MuonPeakLAr.png}
\caption{(Left) The red curve is the normalized intensity distribution for pure liquid argon, while the blue curve normalized intensity distribution for 1 ppm of nitrogen in liquid argon scaled by the max value of the pure liquid argon distribution. (Right)The red(blue) spectrum is a background subtracted muon double coincidence spectrum in pure(1 ppm $N_2$) argon. The fit lines are Landau distributions.} 
\label{fig MuonPeakLAr}
\end{figure}

\subsection{Optical Simulations in BACoN}

The software package Geant4 \cite{Geant4} is used to simulate the light collection efficiencies of scintillation events in BACoN. Geant4 discretizes particle propagation through matter, allowing for a wide range of energies and particles to be accurately modeled. This is possible through a reliance on fundamental physics to dictate how a particle should interact on a step by step basis. When the physics does not accurately model a process or is missing (i.e. neutron or optical processes), Geant4 allows for user input to fill in the missing processes. In order to accurately model optical physics in Geant4, \say{Optical Photons} are used to decouple optical processes from electromagnetic processes that are typically experienced by higher energy gammas. Additionally, due to the optical nature of materials, Geant4 requires users to input their own optical properties. These optical properties include surface reflectivity, attenuation length, scintillation yield, absorption and emission spectra, and Rayleigh scattering lengths. Finally, optical surface properties for every material must be defined in order to accurately model the angular distributions of reflections (Lambertian, Lobe, spike, ect..) \cite{Dietz-Laursonn:2016ree}.

Simulation light yield for the liquid argon detectors requires running radioactive decay simulation (i.e. $\ce{K^{42}}$, Uranium, or Thorium) and optical simulations simultaneously. This requires an extensive amount of CPUs and runtime due to the many discrete steps an optical photon can take. For example, if one were to simulate the thorium decay chain, several MeV of energy are deposited in the liquid argon. For every MeV of energy about 40,000 VUV photons are generated. These photons can then be wavelength shifted and internally reflected through the optical fibers before their tracks terminate. For large experiments like LEGEND, in which the optical fibers are upwards of $\sim$ 2.0 m long, these photons can internally reflect tens of thousands of times before being detected at a SiPM. It quickly becomes obvious that without a dedicated large computing cluster, this task can take a very long time to complete.

\subsection{Optical Heat Maps}

In order to decrease the runtime of these simulations, they are broken into two different simulations. By using the fact that scintillators emit light isotropically and has a scintillation yield that is linear in energy, an optical \say{heat} map can be created that maps the photon detection probability as a function of photon initial position throughout the scintillator volume. Once these maps are created, they provide the average light yield as a function of position without having to run an optical simulation in conjunction with the radioactive decay. Though generating an optical map is quite CPU intensive, it only needs to be done once. Average photon yield, $N$, is calculated as:
\begin{equation}
\label{eq averageLightYield}
N = (Y_{scint})\times(E_{dep}(r))\times(P_{detection}(r))\times(\epsilon_{detector})
\end{equation}
where $Y_{scint}$ is the scintillator light yield, $E_{dep}(r)$ is the energy deposition in the scintillator, $P_{detection}(r)$ is the detection probability, and $\epsilon_{detector}$ is the light detector efficiency. Both the energy deposited and detection probability depend on position which takes into account the discrete nature of how Geant4 tracks particles. The average yield is calculated per step for each particle track and is summed at the end of the event in order to estimate the average light yield of the event.

Liquid argon optical \say{heat} maps are created by generating VUV photons with a mean wavelength of 128 nm and gaussian sigma of 2.93 nm and propagating them through the volume. In order to be counted as detected, these VUV photons have to deposit energy in the optical sensitive volume of the simulation. For both BACoN and LEGEND simulations, the VUV photons must first be wavelength shifted. VUV photons that deposit energy in the optical sensitive volumes are not counted. Photon detection probability is calculated per 5x5x5 mm$^3$ voxel as the number of VUV photons detected from that voxel divided by the total number of VUV photons generated in that voxel. The random vertices are chosen to be in the liquid argon in order to simulate a scintillation event. The photon direction is generated isotropically.

\subsection{BACoN Simulations}

BACoN's optical volumes include gaseous argon, liquid argon, stainless steel, TPB, acrylic and the PMT windows. One PMT was lost prior to obtaining pure liquid argon and thus only one PMT is used as an active volume. All optical properties for LEGEND simulations are summarized in appendix \ref{appen OpticalProperties}. 10 ppm of xenon was simulated. The PMTs are modeled as a stainless steel tube with a height of 6 inches and a diameter of 3.125 inch. The three inch \say{cathode} window is embedded on the top and is simulated as the sensitive optical volume, which means that photons of a given wavelength that enter the volume have a detection efficiency dictated by the assigned quantum efficiency. If a photon is not detected, it does not deposit energy in the cathode. An \sfrac{1}{8} thick acrylic disk covers the cathode, while a 2 $\mu$m thick TPB disk covers the acrylic. 

The liquid argon optical map generated for BACoN can be seen in Figure \ref{fig BACoNOpticalMap} and the xenon doped liquid argon map can be seen in Figure \ref{fig BACoNOpticalMapXeD}. In order to project this three dimensional map into two dimensions, the third dimension is averaged over. The xenon doped liquid argon has had its attenuation length extended from 60.0 cm to 1000.0 m to model its transparency in the VUV. The scintillation wavelength has been shifted from 128 nm to 175 nm and the Gaussian mean has been shifted from 2.93 nm to 8.60 nm. The xenon doped attenuation length has not been measured at these concentrations and thus the 1000.0 m attenuation length is chosen not because it is the physical value but rather because this length is much larger than the length of the cryostat. A study of attenuation length versus muon peak shape is discussed below. The gaseous phase in both maps is argon, which starts at Z = +180 mm and extends to Z = +300 mm. The low vapor pressure of xenon in cold gaseous argon causes the concentration of xenon to be negligible. It can be seen that xenon doped argon allows for improved light collection farther from the PMTs which can be attributed to the increased attenuation length. Both maps have highly non uniform light response thus demonstrating that BACoN will not be able to see peaks from most nuclear decays.

\FloatBarrier
\subsection{Cosmic Muon Simulations}

Cosmic muons were pursued as an alternative to nuclear sources as a way of calibrating the optical maps. Cosmic muons are triggered on by placing two 0.35 x 17.0 x 8.50 inch$^3$ scintillating panels above and below the cryostat and rotating the bottom one by 90$^{\circ}$ relative to the top panel. This double coincidence requirement for the cosmic muon selects muons that are preferentially pointed straight down thus limiting the variance in the possible paths the muon can travel while traversing the argon (Figure \ref{fig muonPaths}). Additionally, muons are minimum ionizing particles with a roughly constant dE/dx of about 2.11 MeV/cm for a 266 MeV muon \cite{PDGCitation}. This energy is deposited uniformly along the muon path, thus allowing for the effects of longer attenuation lengths to be explored. Muons deposit much more energy than nuclear decays and take approximately the same path through the cryostat. This features obfuscates the low light collection issues and the non uniform light response. 
\begin{figure}
\centering
\captionsetup{width=1.0\linewidth}
\includegraphics[width=0.250\linewidth,height=0.25\linewidth]{./Figures/Simulations/muonPaths.png}
\includegraphics[width=0.50\linewidth]{./Figures/Simulations/muonZDirection.png}
\caption{ (left) A ray tracing drawing of the BACoN geometry implemented in Geant4. The minimum and maximum path of the muons are indicated with the green dotted lines. (right) The z direction of muons that pass through both panels.} 
\label{fig muonPaths}
\end{figure}

Muon kinetic energies were generated according to a power law:
\begin{equation}
    KE = \left(E_{0}-E_{cut}\right)\sqrt{1-x} - E_{0}
\end{equation}
where $E_{0}$ is the mean energy and is set to 4 $GeV$, $E_{cut}$ is the minimum kinetic energy of the muon set to 1 $MeV$, and $x$ is a random number from 0 to 1. The downwards momentum was chosen from a $cos^{2}(\theta)$ distribution, while the horizontal momentum was chosen to be uniform. The muons were generated in a disk with a diameter of 40 inches directly above the top muon panel. The simulated energy deposited in the liquid argon can be seen in the plot in Figure \ref{fig muonEdep}. The spectrum has two peaks at 82 MeV and 100 MeV. The double peaked spectrum is due to muons taking the shortest path through the counting well and thus depositing less energy in the liquid and still being in coincidence with the panels. The predicted photo electron spectrum for argon and xenon doped argon can be seen in Figure \ref{fig muonSpectrum}. These spectra have been convolved with the PMT single photon resolution ($\sigma_{SPE}$ = 0.3125 PE). Both spectra were fit to a Landau function and have a most probably value (MPV) at 4235 $\pm$ 46.5 PE and 2138 $\pm$ 24 PE for xenon doped and pure liquid argon respectively. Thus, it is predicted that xenon doped argon should yield BLAH times more light from cosmic muons than pure liquid argon. These peaks will be very distinct from nuclear background decays because of the shape and much larger mean of the spectrum. Additionally, cosmic muons can be a triggered source unlike random nuclear decays.

\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=0.95\linewidth]{./Figures/Simulations/muonEdep.png}
\caption[ Energy deposited in the liquid argon from cosmic muons that are in a double coincidence with the muon panels.]{ Energy deposited in the liquid argon from cosmic muons that are in a double coincidence with the muon panels. The red line is a Gaussian plus a Landau function to model the left and right peaks respectively. The double peak comes from muons pass through the counting and not depositing energy in the liquid argon. } 
\label{fig muonEdep}
\end{figure}

\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=0.495\linewidth]{./Figures/Simulations/muonSpectrumLAr.png}
\includegraphics[width=0.495\linewidth]{./Figures/Simulations/muonSpectrumXeD.png}
\caption[Simulated muon spectrum after the double muon panel coincidence is applied for pure liquid argon and xenon doped liquid argon.]{ Simulated muon spectrum after the double muon panel coincidence is applied for pure liquid argon (left plot in red) and xenon doped liquid argon (right plot in blue). The red line in both plots is a Landau function with a MPV of 2138 and 4269 for the pure liquid argon and xenon doped liquid argon respectively.} 
\label{fig muonSpectrum}
\end{figure}

It will be likely that the MPV for each Landau component in simulation is different than the physical peaks. If the MPV is wrong, the quantum efficiency of the PMT, TPB or scintallator light yield are wrong. If the shape of cosmic muon distribution in data is well described by a Landau fit, it suggests that the simulated liquid argon attenuation length is correct. The attenuation length effects light collection efficiencies exponentially while PMT and TPB quantum efficiencies and scintillator yield effect it linearly. The total light collection efficiency can be calculated as:
\begin{equation}
\label{eq simulation lightYield}
\epsilon_{total} \sim e^{-x/\lambda_{atten}}\cdot \epsilon_{TPB} \cdot \epsilon_{PMT}   \cdot Y_{scint}
\end{equation}
where x is the position of the interaction in the liquid argon, $\lambda_{atten}$ is the liquid argon attenuation length, $\epsilon_{TPB}$ is the TPB quantum efficiency, $\epsilon_{PMT}$ is the PMT quantum efficiency, and $Y_{scint}$ is the scintillator yield. 

In order to understand the effect that the attenuation length has on the shape of the distribution, several xenon doped optical maps were made with varying attenuation lengths. The shape of the distribution is defined as the width of the Landau divided by the MPV. This ratio as a function of xenon doped attenuation can be seen in Table \ref{table muonPeakShape}. It can be seen that below an attenuation length of 5.0 m, the shape begins to signifcantly change. The smallest attenuation length that best estimates the shape of the real data will be used. These simulations will be compared to data from BACoN in Chapter \ref{ch XeD}.


\begin{table}[]
\centering
\begin{tabular}{ |p{2.75cm}||p{3.5cm}|p{3.5cm}|p{3.5cm}|  }
 \hline
 \multicolumn{4}{|c|}{Muon Peak Shape versus Attenuation Length} \\
 \hline
  Attenuation Length (m) & MPV (PE)& Sigma (PE)& Ratio (sigma/MPV) \\
 \hline
 1    & 2786$\pm$14 & 898$\pm$9   & 0.322$\pm$0.0035 \\
 5    & 3911$\pm$18 & 1169$\pm$12 & 0.299$\pm$0.0034  \\
 10   & 4091$\pm$19 & 1201$\pm$13 & 0.293$\pm$0.0034   \\
 20   & 4167$\pm$19 & 1229$\pm$13 & 0.294$\pm$0.0033 \\
 50   & 4114$\pm$19 & 1248$\pm$13 & 0.303$\pm$0.0036  \\
 1000 & 4269$\pm$20 & 1291$\pm$14 & 0.302$\pm$0.0036  \\
 \hline
\end{tabular}
\caption[Summary of muon peak shape versus attenuation length]{Summary of muon peak shape versus attenuation length. Each muon peak was fit with a Landau function and the MPV and sigma were extracted. The errors are the statistical errors from the fits.}
\label{table muonPeakShape}
\end{table}


\subsection{Xenon Doping}
\label{sec XeD}
Results from the Run Two nitrogen doping tests prove that a small quantity of gas can be reliably inserted into the liquid argon volume of BACoN with small uncertainties. Four xenon doping steps were taken, 1$\pm$0.04 ppm, 2$\pm$0.05 ppm, 5$\pm$0.09 ppm, and 10$\pm$0.13 ppm. Xenon was injected in 0.5 ppm steps until the desired molar concentration was reached. Each 0.5 ppm injection takes about 30 minutes and thus high  concentrations of xenon ($\sim$ 100 ppm) were not considered due to the long times involved in doping. Once the concentration was stable and fully mixed, 50,000 events were used for all 4 concentrations to create the scintillation distributions (waveforms) seen in Figure \ref{fig AveragedWaveforms}. Note that after-pulsing is still present. Xenon doping shifts the waveforms to a more xenon like (shorter) time distribution where the after-pulsing is more prominent. The waveforms were fit from 1.05 $\mu$s to 10 $\mu$s in order to fit as much of the waveform as possible while still avoiding fitting the singlet. 
\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=1.0\linewidth]{./Figures/XenonDoping/AveragedWaveforms.png}
\caption[Pulse arrival time weighted by pulse charge for xenon concentrations 1,2,5,and 10 ppm]{Scintillation distributions created by binning pulse arrival times weighted by the pulse charge for various concentrations of xenon from 0 - 10 ppm. Distributions are normalized and then scaled to have the same maximum value. } 
\label{fig AveragedWaveforms}
\end{figure}

A modified version of Equation \ref{eq xenonDoped scint} was used to measure the time constants of the mixture:
\begin{equation}
\label{eq xenonFit}
    r = A_1 e^{-t/T_{s}} - A_2 e^{-t/T_{d}} + A_3 e^{-t/T_{long}} 
\end{equation}
where $T_{s}$ is the slow component, $T_{d}$ is energy transfer time between the xenon and triplet state of the argon, $A_{1}$, $A_{2}$ and $A_{3}$ are the intensities, and $T_{long}$ is an additional time constant to account for the tail at late times. $T_{long}$ accounts for the long exponential at late times and has not been reported in previous xenon doping papers. It is speculated that this long component could be from xenon resonance line at 145 nm as seen in \cite{Heindl_2010}. The slow component $T_s$ represents the time constant for the combination of unquenched argon dimer light and xenon dimer light created through the mechanism outline in Chapter \ref{sec XenonDopingTheory}, Section \ref{section XeD}. Though xenon decays rather quickly compared to argon, the population of xenon dimers is \say{pumped} by the argon xenon mixed state, thus is able to have a much longer decay time. The total concentration of xenon dimers and argon dimers in the triplet state is $A_1 e^{-t/T_{s}} - A_2 e^{-t/T_{d}}$. The fit waveforms can be seen in figure \ref{fig XenonFits}. The results from these fits for all four concentrations are summerized in table \ref{table XeDTimes}. It can be seen that the long component begins to decrease at a concentration of 10 ppm xenon. Additionally, $T_s$ at 10 ppm has not decreased much compared to the $T_s$ measured at 5 ppm xenon (447 ns versus 503 ns) while $T_d$ has dropped by about a factor of two between these two concentrations (213 ns versus 435 ns). This would suggest that the xenon dimer has become the dominate contributor to the $T_s$ state. Additionally, this process would help quench any xenon resonance state that would create this long tail ($T_{long}$) due to the dimer state becomes more likely to be formed. This idea is supported by the spectroscopy results measured by \cite{Neumeier}.


\begin{figure}
\begin{tabular}{cc}
  \includegraphics[width=.450\linewidth]{./Figures/XenonDoping/1ppmXenonFit.png} &
  \includegraphics[width=.450\linewidth]{./Figures/XenonDoping/2ppmXenonFit.png}\\
(a) 1 ppm xenon & (b) 2 ppm \\[6pt]
 \includegraphics[width=.450\linewidth]{./Figures/XenonDoping/5ppmXenonFit.png} &
 \includegraphics[width=.450\linewidth]{./Figures/XenonDoping/10ppmXenonFit.png}\\
(c) 5 ppm & (d) 10 ppm \\[6pt]
\end{tabular}
\caption[Fits for Xenon doping waveforms]{Fit of equation \ref{eq xenonFit} for xenon doped waveforms with xenon concentrations of 1, 2, 5, and 10 ppm. The solid red line is the total fit, the dashed blue line is the long exponential component associated with $T_l$, and the magenta dashed line is the xenon dimer and argon triplet component ($A_1 e^{-t/T_{s}} - A_2 e^{-t/T_{d}}$). Deviations from the fit at short times (1.5-2.5 $\mu$s) are due to }
\label{fig XenonFits}
\end{figure}

\begin{table}[]
\centering
\begin{tabular}{ |p{2.75cm}||p{3.5cm}|p{3.5cm}|p{3.5cm}|  }
 \hline
 \multicolumn{4}{|c|}{Xenon Doping Time Constants} \\
 \hline
  Concentration & $T_{s}$ (ns)& $T_{d}$ (ns)& $T_{long}$ (ns)\\
 \hline
 1 ppm  & 1243$\pm$7$\pm$6    & 871$\pm$10$\pm$4   & 3532$\pm$212$\pm$117  \\
 2 ppm  & 771$\pm$12$\pm$1    & 721$\pm$11$\pm$1   & 3285$\pm$4$\pm$5  \\
 5 ppm  & 503$\pm$11$\pm$1    & 435$\pm$9$\pm$1    & 3415$\pm$3$\pm$19   \\
 10 ppm & 447$\pm$1$\pm$2     & 213$\pm$4$\pm$2    & 2732$\pm$4$\pm$14  \\
 \hline
\end{tabular}
\caption[Summary of xenon doping time constants]{Summary of xenon doping time constants, measured in nanoseconds, for various molar concentration from 1 to 10 ppm xenon. The first error is a systematic error estimated by varying the start time of the fit from 1.025 $\mu$s to 1.05 $\mu$s and the second error is statistical. }
\label{table XeDTimes}
\end{table}

Previous measurements of $T_{s}$ for 1 ppm xenon measure it to be between 1 $\mu$s and 2.5 $\mu$s, though the uncertainty on these past measured concentration is also 1 ppm. While measurements of $T_{s}$ at 10 ppm xenon find it to be between 280 ns and 750 ns, and the uncertainty on the concentration is at least 3 ppm for these measurements. $T_{d}$ has not been measured for 1 ppm of xenon, but for 10 ppm the value ranges from about 250 ns to about 700 ns. These values can be seen in Figures \ref{fig XenonDopingTransfer} and \ref{fig XenonDopingShortLong} in Chapter \ref{sec XenonDopingTheory}. The previous measurements on these time constants have a much larger uncertainty on the xenon concentration and thus should not be used as a benchmark for the data presented in this thesis. Disagreement between previous measurements shown in Figures \ref{fig XenonDopingTransfer} and \ref{fig XenonDopingShortLong} is likely due to this same issue.

\FloatBarrier
\section{Cosmic Muon in BACoN}
Cosmic muons, triggered by two 0.35-inch thick plastic scintillator panels, were used as an alternative triggered source to quantify the increase in light yield from xenon doping. The double coincidence spectrum of cosmic muons seen in 10 ppm xenon in liquid argon is the blue curve in the left plot in Figure \ref{fig MuonPeaksin10ppm}. According to the simulation (Figure \ref{fig muonSpectrum}), there should be no low energy tail to the double coincidence muon spectrum. It was suspected that this tail was due to random coincidences in the two panels, so a double coincidence run was taken where the muon panels were placed next to each other and away from the liquid argon such that a muon was very unlikely to interact in both panels and the liquid. The double coincidence noise spectrum is the red curve in the left plot in Figure \ref{fig MuonPeaksin10ppm}. This noise curve was scaled by the ratio of the max values of the two curves in order to account for a different number of entries in each spectrum. These two spectra were then subtracted from each other in order to obtain a pure double coincidence muon spectrum (right plot in Figure \ref{fig MuonPeaksin10ppm}). A Landau was fit to the curve and a most probable value (MPV) of 604.8 $\pm$ 6.4 PE was extracted. The shape of the distribution (sigma/MPV) is measured to be $0.293 \pm 0.008$.   

In order to best match the data to the correct simulated attenuation length, the shape of the simulated peak (sigma/MPV) must be within one standard deviation of the measured value. The simulation with the lowest attenuation length that matches this criteria is chosen as the best lower limit on the real attenuation length. A plot of attenuation length versus muon peak shape can be seen in Figure \ref{fig AttenuationLength}. It can be seen from the figure that the 5.0 m attenuation length simulation is the lowest attenuation value that still fits the data.

\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=1.0\linewidth]{./Figures/XenonDoping/AttenuationLength.png}
\caption[Simulated attenuation lengths muon peak shape compared to measured peak shape]{ Attenuation length, measured in meters, is plotted against the muon peak shape (sigma/MPV). The blue dashed line represents the measured peak shape value, while the light blue band is the error of the peak shape value. Below attenuation lengths 5.0 m, the simulation is no longer consistent with data. This defines a lower bound on the upper limit of the attenuation length of 175 nm light in 10 ppm xenon in argon.} 
\label{fig AttenuationLength}
\end{figure}

The simulation, using an attenuation length of 5.0 m, predicts a MPV 3911$\pm$18 PE, which is 6.47$\pm0.08$ times more than what is measured in 10 ppm of xenon in liquid argon. If the MPV of the simulated muon spectrum is scaled by the ratio of the measured and simulated MPVs ($\times$6.47) and the simulated spectrum is refit with a Landau function, then a MPV of 595$\pm$3 PE is found while the shape is measured to be 0,306$\pm$0.003 (top right plot in Figure \ref{fig SimDataComparisonXeD}). The MPV and shape parameter are consistent with the measured 604.8 PE for peak seen in 10 ppm xenon in liquid argon. Differences in these two values comes from the low PE tail seen in data, which is likely residual background that was not fully subtracted out. Despite this small difference in the low PE tail, the shape of the simulated spectra is well matched to the measured spectrum (bottom plot in Figure \ref{fig SimDataComparisonXeD}). 

\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=0.49\linewidth]{./Figures/XenonDoping/XeD10ppmMuonSpectrum.png}
\includegraphics[width=0.49\linewidth]{./Figures/XenonDoping/XeD10ppmMuonSpectrumSubtract.png}
\caption{(left) The blue PE spectrum is from cosmic muons in double coincidence in 10 ppm xenon in liquid argon (signal) while the red PE spectrum from random double coincidences events in the muon panels as seen in the liquid (background). (right) A signal minus background double coincidence PE muon spectrum seen in 10 ppm xenon. The red curve is a Landau function with a MPV of 604.8 $\pm$ 6.4 PE and a sigma of 168 $\pm$ 3.6 PE } 
\label{fig MuonPeaksin10ppm}
\end{figure}

\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=0.49\linewidth]{./Figures/XenonDoping/XeD10ppmMuonSpectrumSubtract.png}
\includegraphics[width=0.49\linewidth]{./Figures/XenonDoping/XeD10ppmMuonSpectrumSim.png}
\includegraphics[width=1.0\linewidth]{./Figures/XenonDoping/XeD10ppmMuonSpectrumSimDataComparison.png}
\caption{(Top Left) The red PE spectrum is cosmic muons in double coincidence in 10 ppm xenon in liquid argon. (Top right) The blue PE spectrum is predicted from simulation and scaled by 6.47. The red curves in both top plots are Landau fits with MPVs of 604.8 $\pm$ 6.4 and 595 $\pm$ 3 for the left and right plots respectively. (Bottom) PE spectrum of both the simulated PE muon peak after scaling (blue) and the physical muon PE peak (red). } 
\label{fig SimDataComparisonXeD}
\end{figure}

The large factor of 6.47 between the predicted PE yield and the measured yield for coincident cosmic muons can be understood using equation \ref{eq simulation lightYield}. The largest contribution to this light decrease is likely due to the degradation of the TPB. During Run One, TPB was found coating the walls of the cryostat and PMT bases. There is no reason for this not to happen in Run Two as well, though the cryostat will be sealed for several more months in order to assess the stability of the xenon argon mixture. The light yield of 40 photons per keV could also not be a valid assumption. The authors of \cite{xenonEmission} state that they measure a yield of about 20 photons per keV even though they have pure argon. These authors also admit that they are using a low energy electron beam and a non relativistic effect may be lessening the yield. Finally, the quantum efficiency of the PMTs may have been reduced when the tubes were contaminated with helium. As the electrons avalanche inside the tube, collisions with helium could reduce the total current output by the tubes. It is hard to quantify how much these effects are reducing the light yield or if some effects have been left out. Thus by reproducing the correct muon spectrum by selecting the correct attenuation length and accounting for this factor of 6.47, this measurement validates the optical heat map technique described in Chapter \ref{ch Sim}. 

\FloatBarrier
\section{Light Yield Comparison}

Two different methods were used to measure the total increase in light yield after xenon doping. The first method looks at the average PE spectra from random triggers while measuring the stability of the xenon mixture. The second method measured the relative shift of the muon peak from double coincidence measurements mentioned above. 

The stability of the xenon mixture was measured by triggering at -250 mV ($\sim$ 15 PE). The threshold was set rather high due to the low acquisition rate of the DAQ and if it was set any lower, the spectrum would be dominated by low PE pulses likely from thermal emissions in the PMTs. Events that pass this trigger requirement are likely a random combination of gammas, betas, and alphas mainly from the stainless steel walls and cosmic muons at larger PE values. The true shape of the spectrum is likely a falling exponential for the random background events from the steel and a Landau for the muon peak. The simulated spectrum of a $\ce{^{60}Co}$, as seen in Figure \ref{fig Co60XeD}, is also a falling exponential which would suggest gammas from nuclear decays do not produce peaks. The very low PE events are a combination of glancing muons, electronic noise, and random nuclear decays from the stainless steel. This random trigger spectrum for pure liquid argon and 5 ppm xenon can be seen in the left and right plots of Figure \ref{fig RandomTriggerSpectrum} respectively.
\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=0.95\linewidth]{./Figures/XenonDoping/RandomTriggerSpectrum.png}
\caption{(Left) PE spectrum for pure liquid argon using a random trigger set at $\sim$ 15 PE. (Right) PE spectrum for 5 ppm xenon in liquid argon using a random trigger set at $\sim$ 15 PE } 
\label{fig RandomTriggerSpectrum}
\end{figure}

The average PE value from the spectra for 1 ppm, 2 ppm, and 5 ppm xenon in liquid argon is 1,369 $\pm$ 42 PE while it slightly increased for 10 ppm to 1,493 $\pm$ 39 PE. These averages were taken by finding the average PE value in the range of 10 to 10,000 PE. Below 10 PE is dominated by noise, while above 10,000 PE has very low statistics and high energy muons can skew the distribution. The average PE calculated for pure liquid argon is 882 $\pm$ 30 PE. This yields a 1.55 $\pm$ 0.07 increase in light yield for xenon concentrations of 1-5 ppm and a 1.69 $\pm$ 0.07 increase for 10 ppm xenon. This average yield is consistent with the factor of 1.60 that the simulation predicted from an averaged PE yield of $\ce{^{60}Co}$ before and after xenon doping.

The cosmic muon peak should be able to be seen in the pure liquid argon random trigger spectrum even though the double coincidence measurement was not set up. Though this peak is dominated by cosmic muons, there is an unknown underlying nuclear spectra. Additionally, the cosmic muons that make up this peak do not have the same paths that the double coincident muons have. Figure \ref{fig SimDataComparisonLAr} shows the random trigger spectrum in pure liquid (red histogram) and the simulated double coincident muon spectrum (blue markers). The simulated spectrum has been scaled by the correction factor found in the xenon doping analysis presented above ( $\times$ 6.47). The two solid curves seen in the figures are the Landau fits. The MPV and sigma from the simulated fit (red curve) are found to be 338$\pm$2 and 123$\pm$1 respectively. Though the peak seen in data is dominated by its Landau component, the underlying shape due to nuclear events adds to the uncertainty of the fit. The data spectrum was fit in two different ranges in order to estimate the this uncertainty. The start point was fixed at 150 PE while the end point was varied from 450 to 600 PE. A MPV of 334$\pm$7(syst)$\pm$1(stat) is found, while a sigma of 85$\pm$4(syst)$\pm$1(stat). The MPV found in data is consistent with the MPV estimated from the simulation. The shape of the two spectra do not match and it is not expected that they should because the muon paths are different in simulation and data.

The same scale factor ($\times$ 6.47) was used for both simulated spectra of pure liquid argon and xenon doped liquid argon. Additionally, both simulations were able to reproduce the data. This factor is a physical quantity representing the decreased light collection efficiency regardless of the scintallator used (xenon doped argon or pure liquid argon). Finally, the simulation predicts an increase light yield of 1.83$\pm$0.02 and an increase of 1.81$\pm$0.05 was measured. Muons generate more light than random background events because they create light through out the whole liquid volume thus take full advantage of the longer attenuation length. This comparison between the simulated double coincidence muon spectrum for xenon doped and pure liquid is the final prediction made by these simulations, thus completely validating the simulation techniques used.

\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=1.0\linewidth]{./Figures/XenonDoping/LArMuonSpectrumSimDataComparison.png}
\caption[Comparison of simulated and physical muon peaks measured in BACoN]{A comparison of simulated and physical muon peaks measured in BACoN. The red histogram is real data, while the blue markers are simulated data. The two curves are Landau fits with the red curve being a fit to data and the blue curve being a fit to the simulated data. } 
\label{fig SimDataComparisonLAr}
\end{figure}

\FloatBarrier
\section{Nitrogen Quenching in Xenon Doped Argon}

It is expected that contaminants in xenon doped liquid argon will quench the total light output less than in pure liquid argon. The total scintillation distribution is shifted to shorter times and thus the probability of colliding with contaminants (collisional damping) is assumed to be less likely. To evaluate this assumption, the shift of the muon peak from a double coincidence was measured was used. This quenching effect cannot be modeled using a Birk's law formalism (as shown in \cite{triplet1.26}) because of the energy transfer between the xenon and argon dimer creates a \say{dark} mixed state that does not emit light but still can be quenched. Because this energy transfer process is also quenched, a comparison of quenching constants between pure argon and xenon doped liquid argon is meaningless. Two concentrations of nitrogen were considered, $1 \pm 0.04$ ppm and $9.95 \pm 0.13$ ppm nitrogen (molar concentrations). These nitrogen contamination concentrations were chosen because commercially available research grade liquid argon can be purchases at 99.999$\%$ or 99.9999 $\%$ pure (10 ppm or 1 ppm). 
\begin{table}[]
\centering
\begin{tabular}{ |p{2.75cm}||p{1.8cm}|p{2.25cm}|p{2.5cm}|  }
 \hline
 \multicolumn{4}{|c|}{Xenon Doping Time Constants} \\
 \hline
Concentration & $T_{s}$ (ns)& $T_{d}$ (ns)& $T_{long}$ (ns) \\
 \hline
 0 ppm & 447$\pm$1$\pm$2     & 213$\pm$4$\pm$2    & 2732$\pm$4$\pm$14  \\
 \hline
 1 ppm  & 439$\pm$1$\pm$1     & 185$\pm$3$\pm$2    & 2408$\pm$3$\pm$2  \\
 \hline
 10 ppm & 415$\pm$1$\pm$1     & 116$\pm$11$\pm$12    & 2321$\pm$4$\pm$14  \\
 \hline
\end{tabular}
\caption{Summary of xenon doping time constants for 10 ppm xenon and various concentrations of nitrogen measured in nanoseconds.}
\label{table XeDN2Times}
\end{table}

The xenon doped scintallation time constants were measured and are summerized in Table \ref{table XeDN2Times}. The scintillation distributions for all three nitrogen concentrations (0,1,10 ppm) can be seen in Figure \ref{fig XedN2Waveforms}. All three distributions are normalized and then scaled by the maximum value of the 0 ppm nitrogen measurement. It can be seen at 10 ppm of nitrogen that significant after-pulsing is distorting the scintillation time distribution. The total light yield in 10 ppm of nitrogen is much lower (see below) thus after-pulsing contributes significantly more to the total light seen in the distribution. 

\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=1.0\linewidth]{./Figures/XenonDoping/XedN2Waveforms.png}
\caption{Time distribution intensities for 10 ppm of xenon and 0, 1, and 10 ppm N$_2$ in liquid argon. The blue curve contains 0 ppm N$_2$ and is has an area of 1, the red curve contains $1 \pm 0.04$ ppm N$_2$ and has an area of 0.908, and the green curve contains $9.95 \pm 0.13$ N$_2$ and has an area of 0.770 .} 
\label{fig XedN2Waveforms}
\end{figure}

At 1 ppm of nitrogen and 10 ppm of xenon in liquid argon the muon peak from a double coincidence trigger was found to shift from 604.8 $\pm$ 6.4 PE to 542 $\pm$ 4 PE which corresponds to 10.4$\pm$1\% drop while this drop in liquid argon was measured to be 15.3$\pm$3.1\%. In 10 ppm N$_2$ and 10 ppm Xe in liquid argon the muon peak shifts to 294 $\pm$ 3 PE which is a 51.4$\pm$0.7\% drop in light yield (Figure \ref{fig XeDN2MuonPeak}). 

\begin{figure}
\centering
\captionsetup{width=1\linewidth}
\includegraphics[width=.49\linewidth]{./Figures/XenonDoping/XeDN2MuonPeak1ppmN2.png}
\includegraphics[width=.49\linewidth]{./Figures/XenonDoping/XeDN2MuonPeak10ppmN2.png}
\caption{Double coincidence muon PE spectrum for 10 ppm xenon and 1 ppm (left plot) and 10 ppm (right plot) nitrogen in liquid argon. The blue points are for 1 and 10 ppm nitrogen and 10 ppm xenon, while the red points are for 0 ppm nitrogen and 10 ppm xenon. Fit lines are Landau distributions.} 
\label{fig XeDN2MuonPeak}
\end{figure}

These doping measurements show that xenon doped argon is less sensitive to the total contamination concentration of nitrogen. Unlike other contaminates like nitrogen, xenon atoms will quench the argon triplet and in some characteristic time $T_d$, will re-emit light. This xenon state is less likely to be quenched because, at 10 ppm xenon, $T_d$ is measured to be 213$\pm$6 ns which is much quicker than the argon triplet life time of 1479 ns. Additionally, xenon doped argon, at 10 ppm nitrogen and 10 ppm xenon, has close to the same total light yield from cosmic muons as pure liquid argon (294 P.E versus 338 PE), thus if one were to buy five 9's liquid argon from a commercial vendor and dope it with 10 ppm of xenon, the total light output would be similar to pure liquid argon. It is also worth noting that five 9's commercial grade argon also has other contaminates in it like oxygen, air, carbon monoxide and carbon dioxide all of which have different quenching factors. Finally, it still might be possible to see less quenching at higher xenon concentrations because $T_{d}$ will be shorter.
